TOI-712: a system of adolescent mini-Neptunes extending to the habitable zone

As an all-sky survey, NASA's $TESS$ mission is able to detect the brightest and rarest types of transiting planetary systems, including young planets that enable study of the evolutionary processes that occur within the first billion years. Here, we report the discovery of a young, multi-planet system orbiting the bright K4.5V star, TOI-712 ($V = 10.838$, $M_\star = 0.733_{-0.025}^{+0.026} M_\odot$, $R_\star = 0.674\pm0.016 R_\odot$, $T_{\rm eff} = 4622_{-60}^{+61}$ K). From the $TESS$ light curve, we measure a rotation period of 12.48 days, and derive an age between about $500$ Myr and 1.1 Gyr. The photometric observations reveal three transiting mini-Neptunes ($R_b = 2.049^{+0.12}_{-0.080} R_\oplus$, $R_c = 2.701^{+0.092}_{-0.082} R_\oplus$, $R_d = 2.474^{+0.090}_{-0.082} R_\oplus $), with orbital periods of $P_b = 9.531$ days, $P_c = 51.699$ days, and $P_d = 84.839$ days. After modeling the three-planet system, an additional Earth-sized candidate is identified, TOI-712.05 ($P = 4.32$ days, $R_P = 0.81 \pm 0.11 R_\oplus$). We calculate that the habitable zone falls between 0.339 and 0.844 au (82.7 and 325.3 days), placing TOI-712 d near its inner edge. Among planetary systems harboring temperate planets, TOI-712 ($T = 9.9$) stands out as a relatively young star bright enough to motivate further characterization.

==> TOI-712 Draft (1) 2/affiliations.tex <==
% \newcommand{\cfa}{Center for Astrophysics \rotatebox[origin=c]{-15}{|} Harvard \& Smithsonian, 60 Garden St, Cambridge, MA 02138, USA}
\newcommand{\cfa}{Center for Astrophysics \textbar{} Harvard \& Smithsonian, 60 Garden Street, Cambridge, MA 02138, USA}
% \newcommand{\cfa}{Center for Astrophysics \textbar \ Harvard \& Smithsonian, 60 Garden St, Cambridge, MA 02138, USA}
\newcommand{\umich}{Astronomy Department, University of Michigan, 1085 S University Avenue, Ann Arbor, MI 48109, USA}
\newcommand{\utaustin}{Department of Astronomy, The University of Texas at Austin, Austin, TX 78712, USA}
\newcommand{\MIT}{Department of Physics and Kavli Institute for Astrophysics and Space Research, Massachusetts Institute of Technology, Cambridge, MA 02139, USA}
\newcommand{\eaps}{Department of Earth, Atmospheric, and Planetary Sciences, Massachusetts Institute of Technology, 77 Massachusetts Avenue, Cambridge, MA 02139, USA}
\newcommand{\mitaero}{Department of Aeronautics and Astronautics, Massachusetts Institute of Technology, 125 Massachusetts Avenue, Cambridge, MA 02139, USA}
\newcommand{\uflorida}{Department of Astronomy, University of Florida, 211 Bryant Space Science Center, Gainesville, FL 32611, USA}
\newcommand{\riverside}{Department of Earth Sciences, University of California,
Riverside, CA 92521, USA}
\newcommand{\usq}{Centre for Astrophysics, University of Southern Queensland, West Street, Toowoomba, QLD 4350, Australia}
\newcommand{\ames}{NASA Ames Research Center, Moffett Field, CA, 94035, USA}
\newcommand{\geneva}{Observatoire de l'Universit\'e de Gen\`eve, 51 chemin des Maillettes,
1290 Versoix, Switzerland}
\newcommand{\uw}{Astronomy Department, University of Washington, Seattle, WA 98195, USA}
\newcommand{\warwick}{Deptartment of Physics, University of Warwick, Gibbet Hill Road, Coventry CV4 7AL, UK}
\newcommand{\warwickceh}{Centre for Exoplanets and Habitability, University of Warwick, Gibbet Hill Road, Coventry CV4 7AL, UK}
\newcommand{\princeton}{Department of Astrophysical Sciences, Princeton University, 4 Ivy Lane, Princeton, NJ 08544, USA}
\newcommand{\liegestar}{STAR Institute, Universit\'e de Li\`ege, All\'ee du 6 Ao\^ut 17, B-4000 Li\`ege, Belgium}
\newcommand{\liegeur}{UR Astrobiology, Universit\'e de Li\`ege, 19C All\'ee du 6 Ao\^ut, B-4000 Li\`ege, Belgium}
\newcommand{\vanderbilt}{Department of Physics and Astronomy, Vanderbilt University, Nashville, TN 37235, USA}
\newcommand{\fisk}{Department of Physics, Fisk University, 1000 17th Avenue North, Nashville, TN 37208, USA}
\newcommand{\columbia}{Department of Astronomy, Columbia University, 550 West 120th Street, New York, NY 10027, USA}
\newcommand{\toronto}{Dunlap Institute for Astronomy and Astrophysics, University of Toronto, Ontario M5S 3H4, Canada}
\newcommand{\unc}{Department of Physics and Astronomy, University of North Carolina at Chapel Hill, Chapel Hill, NC 27599, USA}
\newcommand{\iac}{Instituto de Astrof\'isica de Canarias (IAC), E-38205 La Laguna, Tenerife, Spain}
\newcommand{\lalaguna}{Departamento de Astrof\'isica, Universidad de La Laguna (ULL), E-38206 La Laguna, Tenerife, Spain}
\newcommand{\louisville}{Department of Physics and Astronomy, University of Louisville, Louisville, KY 40292, USA}
\newcommand{\aavso}{American Association of Variable Star Observers, 49 Bay State Road, Cambridge, MA 02138, USA}
\newcommand{\utokyo}{Department of Astronomy, The University of Tokyo, 7-3-1 Hongo, Bunky\={o}, Tokyo 113-8654, Japan}
\newcommand{\naoj}{National Astronomical Observatory of Japan, 2-21-1 Osawa, Mitaka, Tokyo 181-8588, Japan}
\newcommand{\jstpresto}{JST, PRESTO, 7-3-1 Hongo, Bunkyo-ku, Tokyo 113-0033, Japan}
\newcommand{\astrobiojapan}{Astrobiology Center, 2-21-1 Osawa, Mitaka, Tokyo 181-8588, Japan}
\newcommand{\ctio}{Cerro Tololo Inter-American Observatory, Casilla 603, La Serena, Chile}
\newcommand{\nexsci}{Caltech/IPAC -- NASA Exoplanet Science Institute 1200 E. California Ave, Pasadena, CA 91125, USA}
\newcommand{\ucsc}{Department of Astronomy and Astrophysics, University of
California, Santa Cruz, CA 95064, USA}
\newcommand{\gsfc}{Exoplanets and Stellar Astrophysics Laboratory, Code 667, NASA Goddard Space Flight Center, Greenbelt, MD 20771, USA}
\newcommand{\sgtinc}{SGT, Inc./NASA AMES Research Center, Mailstop 269-3, Bldg T35C, P.O. Box 1, Moffett Field, CA 94035, USA}
\newcommand{\espace}{Espace, Inc., 30 Lynn Avenue, Hull, MA 02045-2216, USA}
\newcommand{\berkeley}{Astronomy Department, University of California Berkeley, Berkeley, CA 94720-3411, USA}
\newcommand{\brorfelde}{Brorfelde Observatory, Observator Gyldenkernes Vej 7, DK-4340 T\o{}ll\o{}se, Denmark}
\newcommand{\noqsi}{Noqsi Aerospace, Ltd., 15 Blanchard Avenue, Billerica, MA 01821, USA}
\newcommand{\protologic}{Proto-Logic Consulting LLC, Washington, DC 20009, USA}
\newcommand{\scsu}{Department of Physics, Southern Connecticut State University, 501 Crescent Street, New Haven, CT 06515, USA}
\newcommand{\telaviv}{School of Physics and Astronomy, Raymond and Beverly Sackler Faculty of Exact Sciences, Tel Aviv University, Tel Aviv 6997801, Israel}
\newcommand{\dtuspace}{DTU Space, National Space Institute, Technical University of Denmark, Elektrovej 327, DK-2800 Lyngby, Denmark}
\newcommand{\seti}{SETI Institute, 189 Bernardo Avenue, Suite 200, Mountain View, CA 94043, USA}
\newcommand{\swarthmore}{Deptartment of Physics \& Astronomy, Swarthmore College, Swarthmore PA 19081, USA}
\newcommand{\cadiayyad}{Oukaimeden Observatory, High Energy Physics and Astrophysics Laboratory, Cadi Ayyad University, Marrakech, Morocco}
\newcommand{\cavendish}{Cavendish Laboratory, University of Cambridge, JJ Thomson Avenue, Cambridge, CB3 0H3, UK}
\newcommand{\oca}{Universit\'e C\^ote d'Azur, Observatoire de la C\^ote d'Azur, CNRS, Laboratoire Lagrange, Bd de l'Observatoire, CS 34229, 06304 Nice cedex 4, France}

%Insert these before the institution affiliation command
\newcommand{\torres}{\altaffiliation{Juan Carlos Torres Fellow}}
\newcommand{\sagan}{\altaffiliation{NASA Sagan Fellow}}
\newcommand{\hubble}{\altaffiliation{NASA Hubble Fellow}}
\newcommand{\nsfgrfp}{\altaffiliation{NSF Graduate Research Fellow}}
\newcommand{\kavli}{\altaffiliation{Kavli Fellow}}
\newcommand{\esafellow}{\altaffiliation{ESA Research Fellow}}


==> TOI-712 Draft (1) 2/authors.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%
% Direct contributions
%%%%%%%%%%%%%%%%%%%%%%%%

\author[0000-0002-0786-7307]{Sydney Vach}
\affiliation{\cfa}

\author[0000-0002-8964-8377]{Samuel N. Quinn} %Did very little but have to include him
\affiliation{\cfa}

\author[0000-0001-7246-5438]{Andrew Vanderburg} %Light curve
\affiliation{\MIT}

\author[0000-0002-7084-0529]{Stephen R. Kane} %Dynamics
\affiliation{\riverside}

\author[0000-0001-6588-9574]{Karen A.\ Collins} %SG1, FFI NEB analysis of 4.3-day candidate
\affiliation{\cfa}

\author[0000-0001-9811-568X]{Adam L. Kraus} %Friend finder, Hyades sequence
\affiliation{\utaustin}

\author[0000-0002-4891-3517]{George Zhou} %CHIRON analysis
\affiliation{\usq}

\author[0000-0001-8726-3134]{Amber A. Medina}
\affiliation{\utaustin}
%%%%%%%%%%%%%%%%%%%%%%%%
% Other data contributions
%%%%%%%%%%%%%%%%%%%%%%%%

% LCO Authors

%asked to be removed via email Nov 1 ejensen1@swarthmore.edu - LCO Key Project and Scheduling
%\author[0000-0002-4625-7333]{Eric L.\ N.\ Jensen}
%\affiliation{Department of Physics \& Astronomy, Swarthmore College, Swarthmore PA 19081, USA}

%rpschwarz@comcast.net - LCO light curve analysis
\author[0000-0001-8227-1020]{Richard P. Schwarz}
\affiliation{Patashnick Voorheesville Observatory, Voorheesville, NY 12186, USA}

%kcolli3@gmu.edu - LCO light curve analysis
\author[0000-0003-2781-3207]{Kevin I.\ Collins}
\affiliation{George Mason University, 4400 University Drive, Fairfax, VA, 22030 USA}

%dennis@astrodennis.com - LCO light curve analysis
\author[0000-0003-2239-0567]{Dennis M.\ Conti}
\affiliation{American Association of Variable Star Observers, 49 Bay State Road, Cambridge, MA 02138, USA}

%thestockdalefamily@bigpond.com - LCO light curve analysis and Hazelwood observation and analysis
\author[0000-0003-2163-1437]{Chris Stockdale}
\affiliation{Hazelwood Observatory, Australia}

%bobmassey1@gmail.com - LCO light curve analysis
\author[0000-0001-8879-7138]{Bob Massey}
\affil{Villa '39 Observatory, Landers, CA 92285, USA}
 
% olga.suarez@oca.eu - ASTEP
\author{Olga Suarez}
\affiliation{\oca}

% tristan.guillot@oca.eu - ASTEP
\author[0000-0002-7188-8428]{Tristan Guillot}
\affiliation{\oca}

\author[0000-0001-5000-7292]{Djamel Mekarnia}
\affiliation{\oca}

\author[0000-0002-0856-4527]{Lyu Abe}
\affiliation{\oca}

\author[0000-0002-3937-630X]{Georgina Dransfield}
\affiliation{School of Physics \& Astronomy, University of Birmingham, Edgbaston, Birmingham, B15 2TT, UK}

\author[0000-0001-7866-8738]{Nicolas Crouzet}
\affiliation{European Space Agency (ESA), European Space Research and Technology Centre (ESTEC), Keplerlaan 1, 2201 AZ Noordwijk, The Netherlands}

\author[0000-0002-5510-8751]{Amaury H. M. J. Triaud}
\affiliation{School of Physics \& Astronomy, University of Birmingham, Edgbaston, Birmingham, B15 2TT, UK}

\author[0000-0003-3914-3546]{François-Xavier Schmider}
\affiliation{\oca}

\author{Abelkrim Agabi}
\affiliation{\oca}

% \author[0000-0002-1560-4590]{Ivan Bruni}
% \affiliation{INAF OAS, Osservatorio di Astrofisica e Scienza dello Spazio di Bologna via Piero Gobetti 93/3, Bologna, Italy}

\author{Marco Buttu}
\affiliation{ INAF Osservatorio Astronomico di Cagliari, Via della Scienza 5 - 09047 Selargius CA, Italy}

\author[0000-0001-9800-6248]{Elise Furlan}
\affiliation{NASA Exoplanet Science Institute, Caltech/IPAC, Mail Code 100-22, 1200 E. California Blvd., Pasadena, CA 91125, USA}
 
\author[0000-0003-2519-6161]{Crystal~L.~Gnilka}
\affiliation{NASA Exoplanet Science Institute, Caltech/IPAC, Mail Code 100-22, 1200 E. California Blvd., Pasadena, CA 91125, USA}
\affil{\ames}

\author[0000-0002-2532-2853]{Steve B.\ Howell} %Gemini speckle; and Elise Furlan? maybe others, too
\affiliation{\ames}

\author[0000-0002-0619-7639]{Carl Ziegler}
\affiliation{Department of Physics, Engineering and Astronomy, Stephen F. Austin State University, 1936 North St, Nacogdoches, TX 75962, USA}

\author[0000-0001-7124-4094]{C\'{e}sar Brice\~{n}o}
\affiliation{Cerro Tololo Inter-American Observatory/NSF’s NOIRLab, Casilla 603, La Serena, Chile}


\author{Nicholas Law}
\affiliation{Department of Physics and Astronomy, The University of North Carolina at Chapel Hill, Chapel Hill, NC 27599-3255, USA}

\author[0000-0003-3654-1602]{Andrew W. Mann}
\affiliation{Department of Physics and Astronomy, The University of North Carolina at Chapel Hill, Chapel Hill, NC 27599-3255, USA}

% emailed asking to be removed
% \author{Edward~H.~Morgan} 
% \affiliation{\MIT}

\author{Alexander~Rudat}
\affiliation{\MIT}

\author{Knicole~D.~Colon}
\affiliation{\gsfc}

\author[0000-0003-4724-745X]{Mark E. Rose}
\affiliation{\ames}

\author{Michelle Kunimoto}
\affiliation{\MIT}

\author[0000-0002-3164-9086]{Maximilian N. Günther}
\esafellow
\affiliation{European Space Agency (ESA), European Space Research and Technology Centre (ESTEC), Keplerlaan 1, 2201 AZ Noordwijk, The Netherlands}


\author[0000-0002-9003-484X]{David Charbonneau}
\affiliation{\cfa}

\author[0000-0002-5741-3047]{David R. Ciardi}
\affiliation{NASA Exoplanet Science Institute, Caltech/IPAC, Mail Code 100-22, 1200 E. California Blvd., Pasadena, CA 91125, USA}

% \author[0000-0003-3773-5142]{Jason D. Eastman}
% \affiliation{\cfa}

%%%%%%%%%%%%%%%%%%%%%%%%
% TESS Architects
%%%%%%%%%%%%%%%%%%%%%%%%

\author[0000-0003-2058-6662]{George R. Ricker}
\affiliation{\MIT}

\author[0000-0001-6763-6562]{Roland K. Vanderspek}
\affiliation{\MIT}

\author[0000-0001-9911-7388]{David W. Latham}
\affiliation{\cfa}

\author{Sara Seager}
\affiliation{\MIT}
\affiliation{\eaps}
\affiliation{\mitaero}

\author[0000-0002-4265-047X]{Joshua N. Winn}
\affiliation{\princeton}

\author[0000-0002-4715-9460]{Jon M. Jenkins}
\affiliation{\ames}



==> TOI-712 Draft (1) 2/newcommands.tex <==
\newcommand{\bjdtdb}{\ensuremath{\rm {BJD_{TDB}}}}
\newcommand{\feh}{\ensuremath{\left[{\rm Fe}/{\rm H}\right]}}
\newcommand{\mh}{\ensuremath{\left[{\rm m}/{\rm H}\right]}}
\newcommand{\teff}{\ensuremath{T_{\rm eff}}\xspace}
\newcommand{\teq}{\ensuremath{T_{\rm eq}}}
\newcommand{\logg}{\ensuremath{\log g}}
\newcommand\vsini{\ifmmode{v\sin{i_\star}}\else $v\sin{i_\star}$\fi}
\newcommand{\vmac}{\ensuremath{v_{\rm mac}}}
\newcommand\sini{\ifmmode{\sin{i_\star}}\else $\sin{i_\star}$\fi}
\newcommand{\ecosw}{\ensuremath{e\cos{\omega_*}}}
\newcommand{\esinw}{\ensuremath{e\sin{\omega_*}}}
\newcommand{\msun}{\ensuremath{\,M_\Sun}}
\newcommand{\rsun}{\ensuremath{\,R_\Sun}}
\newcommand{\lsun}{\ensuremath{\,L_\Sun}}
\newcommand{\mj}{\ensuremath{\,M_{\rm J}}}
\newcommand{\rj}{\ensuremath{\,R_{\rm J}}}
\newcommand{\rearth}{\ensuremath{\,R_{\rm \Earth}}\xspace}
\newcommand{\mearth}{\ensuremath{\,M_{\rm \Earth}}\xspace}
\newcommand{\re}{\ensuremath{\,R_{\rm \Earth}}\xspace}
\newcommand{\me}{\ensuremath{\,M_{\rm \Earth}}\xspace}
\newcommand{\mb}{\ensuremath{\,M_{\rm b}}}
\newcommand{\mc}{\ensuremath{\,M_{\rm c}}}
\newcommand{\md}{\ensuremath{\,M_{\rm d}}}
\newcommand{\fave}{\langle F \rangle}
\newcommand{\fluxcgs}{10$^9$ erg s$^{-1}$ cm$^{-2}$}
\newcommand{\newln}{\\&\quad\quad{}}
\newcommand{\Kepler}{{\it Kepler}}
\newcommand{\kep}{{\it Kepler}}
\newcommand{\Ktwo}{{\it K2}}
\newcommand{\tess}{{\it TESS}}
\newcommand{\tesspar}{{\it Transiting Exoplanet Survey Satellite} ({\it TESS)}}
\newcommand\mysim{\mathord{\sim}}
\newcommand{\kms}{\,km\,s$^{-1}$}
\newcommand{\ms}{\,m\,s$^{-1}$}
\newcommand{\masyr}{\ensuremath{{\rm mas\,yr}^{-1}}}
\newcommand{\minus}{\scalebox{0.75}[1.0]{$-$}}
\newcommand{\thisstar}{TOI-712\xspace}
\newcommand{\thisstarone}{TOI-712.01\xspace}
\newcommand{\thisstartwo}{TOI-712.02\xspace}
\newcommand{\thisstarthree}{TOI-712.03\xspace}
\newcommand{\thisstarfour}{TOI-712.04\xspace}
\newcommand{\thisstarb}{TOI-712\,b\xspace}
\newcommand{\thisstarc}{TOI-712\,c\xspace}
\newcommand{\thisstard}{TOI-712\,d\xspace}
\newcommand{\thisstare}{TOI-712\,e\xspace}
\newcommand{\thistic}{TIC\,52368076\xspace}
\newcommand{\bradius}{\ensuremath{2.049}}
\newcommand{\bradiuse}{\ensuremath{2.049^{+0.12}_{-0.080}}}
\newcommand{\cradius}{\ensuremath{2.701}}
\newcommand{\cradiuse}{\ensuremath{2.701^{+0.092}_{-0.082}}}
\newcommand{\dradius}{\ensuremath{2.474}}
\newcommand{\dradiuse}{\ensuremath{2.474^{+0.090}_{-0.082}}}
\newcommand{\mstar}{\ensuremath{M_{*}}}
\newcommand{\rstar}{\ensuremath{R_{*}}}
\newcommand{\ar}{\ensuremath{a/R_*}}
\newcommand{\fracbrac}[2]{\left(\frac{#1}{#2}\right)}
\newcommand{\vespa}{{\texttt{vespa}}\xspace}
\newcommand{\rffig}[1]{Fig.~\ref{fig:#1}}
\newcommand{\rffigl}[1]{Figure~\ref{fig:#1}}
\newcommand{\rffigs}[2]{Figures~\ref{fig:#1} and \ref{fig:#2}}
\newcommand{\rfsec}[1]{\mbox{\S\ \ref{sec:#1}}}
\newcommand{\rfsecl}[1]{\mbox{Section \ref{sec:#1}}}
\newcommand{\rfsecs}[2]{\mbox{Sections \ref{sec:#1} and \ref{sec:#2}}}
\newcommand{\rftab}[1]{Tab.~\ref{tab:#1}}
\newcommand{\rftabl}[1]{Table~\ref{tab:#1}}
\newcommand{\rftabs}[2]{Tables~\ref{tab:#1} and \ref{tab:#2}}
\newcommand{\rfeq}[1]{Eq.~\ref{eq:#1}}
\newcommand{\rfeql}[1]{Equation~\ref{eq:#1}}


==> TOI-712 Draft (1) 2/rvtable.tex <==
\begin{deluxetable}{lcc}
\label{tab:rvs}
\tablewidth{\textwidth}
\tablecaption{CHIRON radial velocities of \thisstar}
\tablehead{\colhead{~~~~~~~${\rm BJD_{TDB}}$~~~~~~~} &
           \colhead{~~~~~~~~~~~~RV~~~~~~~~~~~~} &
           \colhead{~~~~~~~~~~~~$\sigma_{\rm RV}$~~~~~~~~~~~~} \\[-1ex]
           \colhead{} &
           \colhead{(\kms)} &
           \colhead{(\kms)}
           }
\startdata
2458746.897310 & 3.822 & 0.064 \\
2458787.812670 & 3.967 & 0.066 \\
2459314.531560 & 3.953 & 0.036 \\
\enddata
\footnotesize{ 
\justifying
\vspace{6pt}
\noindent \textbf{Note.} The CHIRON radial velocities show no significant variation that might have been indicative of a bound stellar companion.}
\vspace{-16pt}
\end{deluxetable}

==> TOI-712 Draft (1) 2/stellar.tex <==
\begin{table}
\scriptsize
\centering
\caption{Literature Properties for \thisstar}
\begin{tabular*}{\columnwidth}{l @{\extracolsep{\fill}} lcr}
  \hline
  \hline
 & \multicolumn{3}{c}{TIC 150151262} \\
Other & \multicolumn{3}{c}{TYC 8905-00810-1} \\
identifiers	  & \multicolumn{3}{c}{2MASS J06114467-6549335} \\
 & \multicolumn{3}{c}{WISE J061144.66-654933.1} \\
\hline
\hline
Parameter & Description & Value & Source\\
\hline 
$\alpha_{J2000}$	&R.A. & 06:11:44.6729007687& 1	\\
$\delta_{J2000}$	&decl. & -65:49:33.499607825& 1	\\
\\
$T$	& \tess\ $T$ mag	& 9.9059 $\pm$ 0.006 & 6	\\
\\
$B_T$	& Tycho $B_T$ mag & 12.10 $\pm$ 0.20		& 2	\\
$V_T$	& Tycho $V_T$ mag & 10.84 $\pm$ 0.07		& 2	\\
$B$\tablenotemark{a}		
        & APASS Johnson $B$ mag	& 11.701 $\pm$	0.025& 3	\\
$V$		& APASS Johnson $V$ mag	& 10.892 $\pm$	0.016& 3	\\
$G$     & {\it Gaia} $G$ mag    & 10.5785 $\pm$ 0.0006    & 1\\
$g'$	& APASS Sloan $g'$ mag	& 11.622 $\pm$ **0.000	& 3	\\
$r'$	& APASS Sloan $r'$ mag	& 10.526 $\pm$ **0.000	& 3	\\
$i'$	& APASS Sloan $i'$ mag	& 10.182 $\pm$ 0.009 & 3	\\
\\
$J$		& 2MASS $J$ mag & 8.984  $\pm$ 0.022	& 4	\\
$H$		& 2MASS $H$ mag & 8.409 $\pm$ 0.042	    & 4	\\
$K_S$	& 2MASS $K_S$ mag & 8.313 $\pm$ 0.023 & 4	\\
\\
\textit{WISE1}		& \textit{WISE1} mag & 8.233 $\pm$ 0.023 	& 5	\\
\textit{WISE2}		& \textit{WISE2} mag & 8.293 $\pm$ 0.020 	& 5 \\
\textit{WISE3}		& \textit{WISE3} mag &8.219 $\pm$ 0.019 	& 5	\\
\textit{WISE4}		& \textit{WISE4} mag & 8.241 $\pm$ 0.127 	& 5	\\
\\
$\mu_{\alpha}$		& PM in R.A. (mas yr$^{-1}$)  & -2.929 $\pm$ 0.047	& 1 \\
$\mu_{\delta}$		& PM in decl. (mas yr$^{-1}$)   	&  31.003 $\pm$ 0.044 &  1 \\
$\pi$ & Parallax (mas)  & 17.0297 $\pm$ 0.0230 & 1 \\
$RV$ & Systemic RV (\kms)   & 3.16 $\pm$ 0.34 & 1 \\
\hline
\\[-6ex]
\end{tabular*}
\begin{flushleft} 
\footnotesize{\vspace{6pt}
    {\bf References.} (1) \citet{GaiaDR22018}; (2) \citet{Hog:2000}; (3) \citet{Henden:2016}; (4) \citet{Cutri:2003}; (5) \citet{Cutri:2014}; (6) \citet{stassun:2018b}
}
\end{flushleft}
\label{tab:stellar}
\end{table}



==> TOI-712 Draft (1) 2/toi712.05.tex <==
\begin{table}
\scriptsize
\centering
\tablewidth{\textwidth}
\caption{Parameters of the candidate TOI-712.05}
\label{tab:toi712_05tab}
\begin{tabular*}{\columnwidth}{l @{\extracolsep{\fill}} l c}
\hline
\hline
Parameter & Description (Units) & Values \\
\hline
$P$  & Period (days) &$4.321298^{+0.000093}_{-0.000069}$\\
$R_P$ & Radius ($R_\oplus$) &$0.81\pm0.11$\\
$R_P / R_*$ & Radius of planet in stellar radii &$0.0110\pm0.0015$\\
$\left(R_P/R_*\right)^2$ & Planet-to-star area ratio &$0.000120^{+0.000035}_{-0.000031}$\\
$\delta_{\rm TESS}$ &Transit depth in TESS band &$0.000122\pm0.000022$\\
$T_C$ & Time of conjunction (BJD$_{\textrm{TDB}}$) &$1388.3796^{+0.0076}_{-0.012}$\\
$a$ & Semi-major axis (AU) &$0.04679^{+0.00041}_{-0.00040}$\\
$a/R_*$ & Semi-major axis in stellar radii &$14.90^{+0.31}_{-0.29}$\\
$i$ & Inclination (Degrees) &$87.09^{+1.1}_{-0.38}$\\
$b$ & Transit impact parameter &$0.757^{+0.093}_{-0.28}$\\
$e$ & Eccentricity & 0.0 (fixed) \\ 
$\omega_*$ & Argument of Periastron (Degrees) & 90.0 (fixed)\\
$T_{14}$ & Total transit duration (hours) &$1.49^{+0.48}_{-0.26}$\\
\hline
\\[-6ex]
\end{tabular*}
\end{table}


==> TOI-712 Draft (1) 2/toi712.lco.tex <==
\begin{deluxetable}{llcl}%[ht]
\label{tab:SG1}
\tablewidth{\textwidth}
\tablecaption{Ground-based transit observations of \thisstar}
\tablehead{\colhead{Date (UT)~~~} &
           \colhead{Telescope~~~} &
           \colhead{Filter~~~}&
           \colhead{Coverage~~~}
           }
\startdata
\multicolumn{4}{l}{\textbf{\thisstarb}} \\
2019-09-11 & LCO-SSO-1.0m & Zs & Egress\\
2019-12-15 & LCO-SAAO-1.0m & Zs & Full\\
2020-01-04 & LCO-SAAO-1.0m & Zs & Full\\
2020-01-23 & LCO-CTIO-1.0m & B & Ingress\\
2020-10-15 & LCO-SAAO-1.0m & B & Full\\
2020-11-13 & LCO-SSO-1.0m & Zs & Full\\
2020-12-12 & LCO-CTIO-1.0m & ip & Full \\\hline
\multicolumn{4}{l}{\textbf{\thisstarc}} \\
2019-12-25$^\dagger$ & LCO-SSO-1.0m & Zs & Egress\\
2019-12-25$^\dagger$ & Hazelwood-0.32m & Rc & Ingress\\
2020-02-15 & LCO-CTIO-1.0m & Zs & Ingress\\
2020-05-28 & ASTEP-0.4m & $\sim$Rc & Full\\
2020-09-09 & LCO-SAAO-1.0m & Zs & Egress\\
2021-04-03 & ASTEP-0.4m & $\sim$Rc & Ingress\\
2021-05-25 & ASTEP-0.4m & $\sim$Rc & Full\\
2021-09-05 & ASTEP-0.4m & $\sim$Rc & Ingress\\
\enddata
\footnotesize{ 
\justifying
\vspace{6pt}
\noindent \textbf{Note.} \noindent $^\dagger$\ indicates an observation that was not used in the global fit. \\[1ex]
The LCOGT filter designations Zs and ip indicate Pan-STARRS $z$-short band and Sloan $i'$ band, respectively. The LCOGT 1\,m telescope nodes used are at Siding Spring Observatory (SSO), Cerro Tololo Inter-American Observatory (CTIO), and South Africa Astronomical Observatory (SAAO). See text regarding the ASTEP observation band.}
\vspace{-16pt}
\end{deluxetable}

==> TOI-712 Draft (1) 2/toi712_ef2.tex <==
\begin{table*}
\scriptsize
\setlength{\tabcolsep}{2pt}
\centering
\caption{\thisstar\ planetary and transit parameters: median values and 68\% confidence intervals}
\begin{tabular*}{\textwidth}{l @{\extracolsep{\fill}} lccc}
  \hline
  \hline
Parameter & Description (Units) & \multicolumn{3}{c}{Values} \\
\hline
\multicolumn{2}{l}{\textbf{Stellar Parameters}}\smallskip\\
~~~~$M_*$\dotfill &Mass (\msun)\dotfill &$0.732^{+0.027}_{-0.025}$\\
~~~~$R_*$\dotfill &Radius (\rsun)\dotfill &$0.674^{+0.017}_{-0.016}$\\
~~~~$L_*$\dotfill &Luminosity (\lsun)\dotfill &$0.1871\pm0.0061$\\
~~~~$\rho_*$\dotfill &Density (cgs)\dotfill &$3.36^{+0.24}_{-0.22}$\\
~~~~$\log{g}$\dotfill &Surface gravity (cgs)\dotfill &$4.645^{+0.021}_{-0.022}$\\
~~~~$T_{\rm eff}$\dotfill &Effective Temperature (K)\dotfill &$4622^{+61}_{-59}$\\
~~~~$[{\rm Fe/H}]$\dotfill &Metallicity (dex)\dotfill &$-0.020^{+0.12}_{-0.043}$\\
~~~~$Age$\dotfill &Age (Gyr)\dotfill &$0.83^{+0.25}_{-0.28}$\\
~~~~$EEP$\dotfill &Equal Evolutionary Phase$^{1}$ \dotfill &$271.4^{+7.8}_{-13}$\\
~~~~$A_V$\dotfill &V-band extinction (mag)\dotfill &$0.083^{+0.049}_{-0.052}$\\
~~~~$\sigma_{SED}$\dotfill &SED photometry error scaling \dotfill &$1.11^{+0.40}_{-0.26}$\\
~~~~$\varpi$\dotfill &Parallax (mas)\dotfill &$17.059\pm0.032$\\
~~~~$d$\dotfill &Distance (pc)\dotfill &$58.62\pm0.11$\\
[1ex]
\hline
\multicolumn{2}{l}{\textbf{Planetary Parameters}} & b & c & d \smallskip\\
~~~~$P$\dotfill &Period (days)\dotfill &$9.531361^{+0.000018}_{-0.000017}$&$51.69906\pm0.00017$&$84.83960^{+0.00043}_{-0.00040}$\\
~~~~$R_P$\dotfill &Radius (\re)\dotfill &$2.049^{+0.12}_{-0.080}$&$2.701^{+0.092}_{-0.082}$&$2.474^{+0.090}_{-0.082}$\\
~~~~$R_P/R_*$\dotfill &Radius of planet in stellar radii \dotfill &$0.02772^{+0.0018}_{-0.00076}$&$0.03669^{+0.00074}_{-0.00059}$&$0.03362^{+0.00079}_{-0.00074}$\\
~~~~$\delta$\dotfill &Transit depth (fraction) \dotfill &$0.000768^{+0.00010}_{-0.000042}$&$0.001346^{+0.000055}_{-0.000043}$&$0.001130^{+0.000053}_{-0.000049}$\\
~~~~$T_C$\dotfill &Time of conjunction$^{2}$ (\bjdtdb)\dotfill &$1385.5457^{+0.0012}_{-0.0010}$&$1429.4054^{+0.0019}_{-0.0017}$&$1470.8665^{+0.0023}_{-0.0025}$\\
~~~~$T_0$\dotfill &Optimal conjunction Time$^{3}$ (\bjdtdb)\dotfill &$1757.26886^{+0.00068}_{-0.00059}$&$1946.39598^{+0.00093}_{-0.00082}$&$1640.5457\pm0.0019$\\
~~~~$T_P$\dotfill &Time of Periastron (\bjdtdb)\dotfill &$1385.49^{+0.43}_{-0.35}$&$1425^{+11}_{-15}$&$1396^{+32}_{-22}$\\
~~~~$T_S$\dotfill &Time of eclipse (\bjdtdb)\dotfill &$1380.9^{+3.5}_{-3.6}$&$1403.6\pm3.2$&$1513.3^{+3.9}_{-3.8}$\\
~~~~$a$\dotfill &Semi-major axis (AU)\dotfill &$0.07928^{+0.00096}_{-0.00091}$&$0.2447^{+0.0030}_{-0.0028}$&$0.3405^{+0.0041}_{-0.0039}$\\
~~~~$i$\dotfill &Inclination (Degrees)\dotfill &$88.22^{+1.1}_{-0.53}$&$89.78^{+0.14}_{-0.11}$&$89.817^{+0.11}_{-0.066}$\\
~~~~$b$\dotfill &Transit Impact parameter \dotfill &$0.41^{+0.32}_{-0.28}$&$0.28^{+0.16}_{-0.19}$&$0.34^{+0.14}_{-0.21}$\\
~~~~$e$\dotfill &Eccentricity \dotfill &$0.54^{+0.26}_{-0.20}$&$0.089^{+0.083}_{-0.056}$&$0.073^{+0.064}_{-0.049}$\\
~~~~$\omega_*$\dotfill &Argument of Periastron (Degrees)\dotfill &$68^{+88}_{-77}$&$115^{+96}_{-95}$&$30^{+110}_{-140}$\\
~~~~$e\cos{\omega_*}$\dotfill & \dotfill &$0.02^{+0.61}_{-0.62}$&$0.001\pm0.097$&$-0.000^{+0.072}_{-0.070}$\\
~~~~$e\sin{\omega_*}$\dotfill & \dotfill &$0.21^{+0.21}_{-0.33}$&$0.029^{+0.046}_{-0.056}$&$0.011\pm0.054$\\
~~~~$\tau$\dotfill &Ingress/egress transit duration (minutes)\dotfill &$3.33^{+2.88}_{-0.56}$&$11.12^{+1.87}_{-0.86}$&$12.5^{+2.0}_{-1.3}$\\
~~~~$T_{14}$\dotfill &Total transit duration (hours)\dotfill &$1.735^{+0.046}_{-0.031}$&$4.843^{+0.058}_{-0.062}$&$5.702^{+0.098}_{-0.094}$\\
~~~~$T_{FWHM}$\dotfill &FWHM transit duration (hours)\dotfill &$1.670^{+0.026}_{-0.024}$&$4.649^{+0.060}_{-0.062}$&$5.486^{+0.101}_{-0.096}$\\
~~~~$\fave$\dotfill &Incident Flux (\fluxcgs)\dotfill &$0.0307^{+0.0056}_{-0.0074}$&$0.00419\pm0.00017$&$0.002176^{+0.000083}_{-0.000080}$\\
~~~~$T_{eq}$\dotfill &Equilibrium temperature$^{4}$ (K)\dotfill &$650.0^{+6.0}_{-5.9}$&$369.9^{+3.4}_{-3.3}$&$313.6^{+2.9}_{-2.8}$\\
~~~~$M_P$\dotfill &Predicted mass$^{5}$ (\me)\dotfill &$5.6^{+2.0}_{-1.3}$&$8.7^{+3.1}_{-1.9}$&$7.5^{+2.7}_{-1.7}$\\
~~~~$M_P/M_*$\dotfill &Predicted mass ratio$^{5}$ \dotfill &$0.0000231^{+0.0000082}_{-0.0000055}$&$0.0000357^{+0.000013}_{-0.0000080}$&$0.0000310^{+0.000011}_{-0.0000072}$\\
~~~~$K$\dotfill &Predicted RV semi-amplitude$^{5}$ (m/s)\dotfill &$2.65^{+1.3}_{-0.72}$&$1.85^{+0.65}_{-0.41}$&$1.36^{+0.48}_{-0.31}$\\
~~~~$\rho_P$\dotfill &Predicted density$^{5}$ (cgs)\dotfill &$3.53^{+1.2}_{-0.84}$&$2.42^{+0.83}_{-0.55}$&$2.73^{+0.95}_{-0.61}$\\
~~~~$logg_P$\dotfill &Predicted surface gravity$^{5}$ \dotfill &$3.11^{+0.13}_{-0.11}$&$3.07^{+0.13}_{-0.11}$&$3.08^{+0.13}_{-0.11}$\\
[1ex]
\hline
\multicolumn{2}{l}{\textbf{Wavelength Parameters}}&TESS\smallskip\\
~~~~$u_{1}$\dotfill &linear limb-darkening coeff \dotfill &$0.463^{+0.043}_{-0.047}$\\
~~~~$u_{2}$\dotfill &quadratic limb-darkening coeff \dotfill &$0.163^{+0.049}_{-0.046}$\\
% ~~~~$A_D$\dotfill &Dilution from neighboring stars \dotfill &$0.0000\pm0.0020$\\
[1ex]
\hline
\multicolumn{2}{l}{\textbf{Transit Parameters}}&\tess\smallskip\\ %May want to characterize each Sector
~~~~$\sigma^{2}$\dotfill &Added Variance \dotfill &$3.29\times10^{-7}\pm0.78\times10^{-7}$\\
~~~~$F_0$\dotfill &Baseline flux \dotfill &$0.9999793\pm0.0000062$\\
[1ex]
\hline \\[-6ex]
\end{tabular*}
\begin{flushleft} 
\footnotesize{\vspace{6pt}{\bf Note---}\\[0.25ex]
$^1$\ Corresponds to static points in a star's evolutionary history. See \S2 in \citet{Dotter:2016}.\\[0.25ex]
$^2$\ Though the time of minimum projected separation is a more correct "transit time, time of conjunction is commonly reported as the transit time, and is in practice identical in all but the most extreme combinations of eccentricity and viewing angles \citep[see][]{Eastman:2019}.\\[0.25ex]
$^3$\ Optimal time of conjunction minimizes the covariance between $T_C$ and Period.\\[0.25ex]
$^4$\ Assumes no albedo and perfect redistribution, making this identical to a surface-averaged irradiation temperature. \\[0.25ex]
$^5$\ Uses measured radius and estimated mass from \citet{Chen:2017}.
}
\end{flushleft}
\label{tab:exofast}
\end{table*}
